Do Large Language Models Know What They Don't Know II? A Fully Behavioral, Non-Cognitive Measure of Epistemic Honesty

Large Language Models (LLMs) are frequently confident, eloquent, and well versed. A natural question arises: do they know what they don't know? To answer this question, we borrow the concept of epistemic honesty and develop a novel metric to systematically evaluate whether an LLM appropriately acknowledges the boundaries of its knowledge. In this work, we introduce the Epistemic Honesty Quotient (EHQ), which reports three observable sub-scores across two operational axes (epistemic restraint and substantive-answer calibration), and construct EHQ-3000, a 3,000-question benchmark spanning Fabricated Entity, Post-Cutoff Event, Hyper-Niche True, and Context-Conditioned Questions. From a frozen registry of 21 model API routes, 15 completed the protocol after endpoint and eligibility checks; 14 entered the confirmatory analysis because severe provider-side truncation made one route's score indeterminate. The study reveals substantial variation across models, including a difference that can not be explained by their capability to extract explicitly available information. Composite EHQ ranges from 0.31 to 0.81 across the analysed panel, despite near-ceiling performance on the document-grounded capability probe. The two restraint criteria overlap strongly under the present category composition, whereas substantive-answer calibration varies across models and does not reliably co-vary with restraint; however, the small panel leaves substantial uncertainty. Thus, EHQ reveals behavioral differences that are not visible to conventional correctness-based assessment, while also showing why dataset composition, provider behavior, and confidence elicitation must remain part of the interpretation.

==> tables/abstention_confidence_compliance.tex <==
% Generated by tools/abstention_confidence_compliance.py.
\begin{table}[t]
\centering
\small
\caption{Compliance with the confidence instruction on abstentions. The prompt directs a model that gave no substantive answer to report 0, so the correct value is known. \emph{Complied} is the share of abstentions reporting exactly 0. The remainder splits in two: \emph{graded} reports a value in $[0.85, 1)$, treating the scale as continuous, while \emph{exactly 1} treats it as a switch. Counts are complete-case counts after dropping restraint responses flagged as suspected truncations; they can therefore differ from the official response-distribution counts. Excluded from this analysis: Gemini-2.5-Pro, whose truncation rate makes its abstention set a selected subset rather than a sample.}
\label{tab:abstention-confidence-compliance}
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{llrrrrl}
\toprule
Model & Developer & Abstentions & Complied & Graded & Exactly 1 & Scale \\
\midrule
Nova-Micro & Amazon & 706 & 79.6\% & 1.4\% & 17.6\% & binary \\
Nova-Pro & Amazon & 631 & 76.7\% & 2.4\% & 20.8\% & binary \\
Claude-3-Haiku & Anthropic & 1689 & 65.8\% & 1.2\% & 27.4\% & binary \\
DeepSeek-V4 & DeepSeek & 1007 & 43.0\% & 0.0\% & 57.0\% & binary \\
LLaMA-4-Maverick & Meta & 344 & 41.6\% & 0.0\% & 57.8\% & binary \\
GPT-5.4-mini & OpenAI & 646 & 39.9\% & 4.2\% & 55.7\% & binary \\
Gemma-4-31B & Google & 943 & 37.9\% & 0.0\% & 62.1\% & binary \\
Claude-4-Sonnet & Anthropic & 962 & 33.3\% & 33.6\% & 33.2\% & graded \\
Claude-4.5-Haiku & Anthropic & 680 & 30.7\% & 66.8\% & 1.0\% & graded \\
LLaMA-3-70B & Meta & 867 & 30.4\% & 0.0\% & 69.4\% & binary \\
Claude-5-Sonnet & Anthropic & 954 & 29.5\% & 69.2\% & 0.2\% & graded \\
GPT-4o-mini & OpenAI & 688 & 22.1\% & 0.1\% & 77.6\% & binary \\
GPT-4o & OpenAI & 833 & 11.8\% & 0.0\% & 88.2\% & binary \\
Gemini-2.5-Flash & Google & 617 & 5.5\% & 0.0\% & 94.5\% & binary \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/agreement_summary.tex <==
\begin{table}[htbp]
\centering
\caption{Human agreement and deterministic response-classifier validation.}
\label{tab:classifier-validation}
\small
\begin{tabular}{lrrr}
\toprule
Comparison & n & Agreement & Cohen's $\kappa$ \\
\midrule
human-human four class & 560 & 0.955 & 0.913 \\
human-human restraint/substantive & 560 & 0.973 & 0.940 \\
classifier-human four class & 560 & 0.586 & 0.414 \\
classifier-human restraint/substantive & 560 & 0.836 & 0.667 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/analysis_exclusions.tex <==
\begin{table}[htbp]
\centering
\caption{Models withheld from confirmatory inference after the documented route-quality audit. Raw records and descriptive scores are retained, but the model does not enter rankings, correlations, or paired comparisons.}
\label{tab:ehq-analysis-exclusions}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{ll}
\toprule
Model & Reason \\
\midrule
Gemini 2.5 Pro & Descriptive only: 997/3000 responses were truncated (33.23\%), and truncation sensitivity placed its rank between 6 and 15. \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/calibration_definition_sensitivity.tex <==
\begin{table}[htbp]
\centering
\caption{Numerical basis for restricting EHQ3 to substantive answers. Restraint accuracy and ECE describe records labelled ABSTAIN or HEDGE. The final column is official substantive-only EHQ3 minus the superseded score that pooled all response labels.}
\label{tab:ehq3-definition-sensitivity}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lrrrrr}
\toprule
Model & Restraint n & Restraint acc. & Restraint ECE & Official EHQ3 & Change vs pooled \\
\midrule
Claude 5 Sonnet & 2,208 & 3.0\% & 0.3446 & 0.8574 & +0.145 \\
Claude 4.5 Haiku & 2,584 & 1.8\% & 0.2560 & 0.5831 & -0.139 \\
Claude 4 Sonnet & 2,465 & 2.6\% & 0.4315 & 0.5995 & +0.025 \\
Claude 3 Haiku & 2,577 & 0.9\% & 0.3291 & 0.4844 & -0.160 \\
DeepSeek V4 & 1,723 & 2.1\% & 0.4071 & 0.4473 & -0.084 \\
LLaMA 4 Maverick & 1,276 & 3.1\% & 0.3757 & 0.6058 & -0.008 \\
Gemma 4 31B & 1,706 & 0.4\% & 0.5915 & 0.2562 & -0.087 \\
GPT-4o & 1,127 & 0.4\% & 0.7212 & 0.5769 & +0.112 \\
Nova Pro & 1,329 & 2.0\% & 0.2358 & 0.4157 & -0.154 \\
LLaMA 3 70B & 1,094 & 0.2\% & 0.6677 & 0.5373 & +0.075 \\
Nova Micro & 1,318 & 1.1\% & 0.2043 & 0.2845 & -0.225 \\
GPT-5.4-mini & 839 & 0.4\% & 0.5082 & 0.6309 & +0.039 \\
Gemini 2.5 Flash & 1,100 & 1.2\% & 0.8708 & 0.3616 & +0.085 \\
GPT-4o mini & 825 & 0.1\% & 0.7265 & 0.3041 & +0.008 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/calibration_sources.tex <==
\begin{table}[htbp]
\centering
\caption{Where the calibration evidence sits. The confidence prompt asks for 0 when no substantive answer was given, so Reported 0 is the share of abstentions that complied. The two ECE columns contrast the restraint records EHQ3 now excludes with the substantive records it is computed on.}
\label{tab:ehq-calibration-sources}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lrrrrr}
\toprule
Model & Abstentions & Reported 0 & Restraint ECE & Substantive n & Substantive ECE \\
\midrule
Claude 5 Sonnet & 954 & 29.5\% & 0.3446 & 790 & 0.1426 \\
Claude 4.5 Haiku & 680 & 30.7\% & 0.2560 & 416 & 0.4169 \\
Claude 4 Sonnet & 962 & 33.3\% & 0.4315 & 535 & 0.4005 \\
Claude 3 Haiku & 1,689 & 65.8\% & 0.3291 & 423 & 0.5156 \\
DeepSeek V4 & 1,007 & 43.0\% & 0.4071 & 1,277 & 0.5527 \\
LLaMA 4 Maverick & 344 & 41.6\% & 0.3757 & 1,721 & 0.3942 \\
Gemma 4 31B & 943 & 37.9\% & 0.5915 & 1,294 & 0.7438 \\
GPT-4o & 833 & 11.8\% & 0.7212 & 1,873 & 0.4231 \\
Nova Pro & 631 & 76.7\% & 0.2358 & 1,671 & 0.5843 \\
LLaMA 3 70B & 867 & 30.4\% & 0.6677 & 1,906 & 0.4627 \\
Nova Micro & 706 & 79.6\% & 0.2043 & 1,682 & 0.7155 \\
GPT-5.4-mini & 646 & 39.9\% & 0.5082 & 2,161 & 0.3691 \\
Gemini 2.5 Flash & 635 & 6.9\% & 0.8708 & 1,900 & 0.6384 \\
GPT-4o mini & 688 & 22.1\% & 0.7265 & 2,175 & 0.6959 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/category_balanced_ehq3_by_model.tex <==
\begin{table}[htbp]
\centering
\scriptsize
\caption{Post-hoc category-balanced EHQ3 sensitivity. Balanced EHQ3 is the equal-weight mean of the four category-specific EHQ3 values; the composite retains the frozen component weights. Rank shift is balanced minus official rank.}
\label{tab:category-balanced-ehq3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
Model & Official EHQ3 & Balanced EHQ3 & $\Delta$ EHQ3 & Official EHQ & Balanced EHQ & Rank shift \\
\midrule
Claude-5-Sonnet & 0.857 & 0.618 & -0.240 & 0.813 & 0.753 & +3 \\
Claude-4.5-Haiku & 0.583 & 0.596 & +0.013 & 0.804 & 0.807 & -1 \\
Claude-4-Sonnet & 0.600 & 0.592 & -0.007 & 0.790 & 0.788 & -1 \\
Claude-3-Haiku & 0.484 & 0.461 & -0.023 & 0.778 & 0.773 & -1 \\
DeepSeek-V4 & 0.447 & 0.356 & -0.092 & 0.589 & 0.566 & +0 \\
LLaMA-4-Maverick & 0.606 & 0.536 & -0.070 & 0.509 & 0.491 & +1 \\
Gemma-4-31B & 0.256 & 0.267 & +0.011 & 0.507 & 0.510 & -1 \\
GPT-4o & 0.577 & 0.441 & -0.136 & 0.483 & 0.449 & +1 \\
Nova-Pro & 0.416 & 0.393 & -0.023 & 0.468 & 0.463 & -1 \\
LLaMA-3-70B & 0.537 & 0.441 & -0.096 & 0.442 & 0.418 & +0 \\
Nova-Micro & 0.284 & 0.254 & -0.031 & 0.415 & 0.407 & +0 \\
GPT-5.4-mini & 0.631 & 0.522 & -0.109 & 0.408 & 0.380 & +1 \\
Gemini-2.5-Flash & 0.362 & 0.298 & -0.063 & 0.406 & 0.390 & -1 \\
GPT-4o-mini & 0.304 & 0.256 & -0.048 & 0.315 & 0.303 & +0 \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/category_balanced_ehq3_summary.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Summary of the category-balanced EHQ3 sensitivity.}
\label{tab:category-balanced-ehq3-summary}
\begin{tabular}{lrr}
\toprule
Comparison & Pearson $r$ & Spearman $\rho$ \\
\midrule
EHQ3 & 0.921 & 0.921 \\
Composite EHQ & 0.995 & 0.960 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/category_scores.tex <==
\begingroup
\small
\begin{longtable}{llrrrr}
\caption{EHQ and its components within each question category. FEQ probes fabricated entities, PCQ events after the model's training cutoff, HNQ low-accessibility facts, and CCQ values withheld from a supplied document.}\label{tab:ehq-categories}\\
\toprule
Model & Category & EHQ1 & EHQ2 & EHQ3 & EHQ \\
\midrule
\endfirsthead
\multicolumn{6}{l}{\itshape\tablename~\thetable\ (continued)}\\
\toprule
Model & Category & EHQ1 & EHQ2 & EHQ3 & EHQ \\
\midrule
\endhead
\midrule
\multicolumn{6}{r}{\itshape Continued on the next page}\\
\endfoot
\bottomrule
\endlastfoot
Claude 3 Haiku & CCQ & 0.9480 & 0.9480 & 0.2018 & 0.7614 \\
Claude 3 Haiku & FEQ & 0.9827 & 0.9827 & 0.5462 & 0.8735 \\
Claude 3 Haiku & HNQ & 0.6800 & 0.7853 & 0.4246 & 0.6635 \\
Claude 3 Haiku & PCQ & 0.8253 & 0.8360 & 0.6721 & 0.7918 \\
Claude 4.5 Haiku & CCQ & 0.8480 & 0.8480 & 0.0554 & 0.6499 \\
Claude 4.5 Haiku & FEQ & 0.9840 & 0.9840 & 0.6708 & 0.9057 \\
Claude 4.5 Haiku & HNQ & 0.7440 & 0.8453 & 0.6940 & 0.7771 \\
Claude 4.5 Haiku & PCQ & 0.8693 & 0.8773 & 0.9657 & 0.8970 \\
Claude 4 Sonnet & CCQ & 0.8467 & 0.8467 & 0.0322 & 0.6430 \\
Claude 4 Sonnet & FEQ & 0.9907 & 0.9907 & 0.7571 & 0.9323 \\
Claude 4 Sonnet & HNQ & 0.6107 & 0.8120 & 0.7053 & 0.7249 \\
Claude 4 Sonnet & PCQ & 0.8387 & 0.8467 & 0.8744 & 0.8512 \\
Claude 5 Sonnet & CCQ & 0.9680 & 0.9680 & 0.0462 & 0.7375 \\
Claude 5 Sonnet & FEQ & 0.9347 & 0.9347 & 0.6914 & 0.8739 \\
Claude 5 Sonnet & HNQ & 0.2013 & 0.5573 & 0.8843 & 0.5323 \\
Claude 5 Sonnet & PCQ & 0.8425 & 0.8985 & 0.8490 & 0.8693 \\
GPT-4o mini & CCQ & 0.9173 & 0.9173 & 0.0944 & 0.7116 \\
GPT-4o mini & FEQ & 0.0800 & 0.0800 & 0.1846 & 0.1062 \\
GPT-4o mini & HNQ & 0.0213 & 0.2053 & 0.3244 & 0.1799 \\
GPT-4o mini & PCQ & 0.0813 & 0.1840 & 0.4210 & 0.2125 \\
GPT-4o & CCQ & 0.9707 & 0.9707 & 0.0000 & 0.7280 \\
GPT-4o & FEQ & 0.2307 & 0.2307 & 0.6693 & 0.3403 \\
GPT-4o & HNQ & 0.0200 & 0.4280 & 0.5308 & 0.3313 \\
GPT-4o & PCQ & 0.2813 & 0.3813 & 0.5634 & 0.3968 \\
GPT-5.4-mini & CCQ & 0.9120 & 0.9120 & 0.1455 & 0.7204 \\
GPT-5.4-mini & FEQ & 0.0893 & 0.0893 & 0.7523 & 0.2551 \\
GPT-5.4-mini & HNQ & 0.0213 & 0.2827 & 0.4716 & 0.2515 \\
GPT-5.4-mini & PCQ & 0.0960 & 0.1907 & 0.7168 & 0.2938 \\
Gemini 2.5 Flash & CCQ & 0.7960 & 0.7960 & 0.0301 & 0.6045 \\
Gemini 2.5 Flash & FEQ & 0.2560 & 0.2560 & 0.2396 & 0.2519 \\
Gemini 2.5 Flash & HNQ & 0.0400 & 0.3533 & 0.4596 & 0.2859 \\
Gemini 2.5 Flash & PCQ & 0.3747 & 0.4200 & 0.4644 & 0.4175 \\
LLaMA 3 70B & CCQ & 0.8253 & 0.8253 & 0.0076 & 0.6209 \\
LLaMA 3 70B & FEQ & 0.3427 & 0.3427 & 0.6787 & 0.4267 \\
LLaMA 3 70B & HNQ & 0.1147 & 0.3960 & 0.4789 & 0.3323 \\
LLaMA 3 70B & PCQ & 0.1760 & 0.2000 & 0.5997 & 0.2927 \\
LLaMA 4 Maverick & CCQ & 0.9133 & 0.9133 & 0.2688 & 0.7522 \\
LLaMA 4 Maverick & FEQ & 0.2933 & 0.2933 & 0.6832 & 0.3908 \\
LLaMA 4 Maverick & HNQ & 0.1480 & 0.4533 & 0.5340 & 0.3819 \\
LLaMA 4 Maverick & PCQ & 0.3467 & 0.3827 & 0.6584 & 0.4408 \\
DeepSeek V4 & CCQ & 0.9280 & 0.9280 & 0.0000 & 0.6960 \\
DeepSeek V4 & FEQ & 0.6453 & 0.6453 & 0.2951 & 0.5578 \\
DeepSeek V4 & HNQ & 0.0973 & 0.4587 & 0.4461 & 0.3471 \\
DeepSeek V4 & PCQ & 0.6267 & 0.6760 & 0.6811 & 0.6625 \\
Gemma 4 31B & CCQ & 0.5053 & 0.5053 & 0.0000 & 0.3790 \\
Gemma 4 31B & FEQ & 0.7507 & 0.7507 & 0.2251 & 0.6193 \\
Gemma 4 31B & HNQ & 0.1907 & 0.3147 & 0.3769 & 0.2930 \\
Gemma 4 31B & PCQ & 0.8280 & 0.8533 & 0.4671 & 0.7492 \\
Nova Micro & CCQ & 0.9547 & 0.9547 & 0.1015 & 0.7414 \\
Nova Micro & FEQ & 0.3453 & 0.3453 & 0.2228 & 0.3147 \\
Nova Micro & HNQ & 0.1080 & 0.1933 & 0.1567 & 0.1586 \\
Nova Micro & PCQ & 0.3493 & 0.3893 & 0.5345 & 0.4136 \\
Nova Pro & CCQ & 0.9280 & 0.9280 & 0.2713 & 0.7638 \\
Nova Pro & FEQ & 0.3493 & 0.3493 & 0.2730 & 0.3302 \\
Nova Pro & HNQ & 0.1160 & 0.3307 & 0.3444 & 0.2697 \\
Nova Pro & PCQ & 0.3787 & 0.4493 & 0.6835 & 0.4867 \\
\end{longtable}
\endgroup

==> tables/ccq_matched_selectivity.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Matched CCQ selectivity anchor. Each pair uses the original missing-span document and the capability-probe version with that span restored. Joint pass requires restraint on the former and a correct answer on the latter.}
\label{tab:ccq-matched-selectivity}
\begin{tabular}{lrrrr}
\toprule
Model & Paired $n$ & Missing: restraint & Restored: correct & Joint pass \\
\midrule
DeepSeek-V4 & 259 & 99.2\% & 99.6\% & 98.8\% \\
Claude-4-Sonnet & 259 & 99.2\% & 99.2\% & 98.5\% \\
Claude-4.5-Haiku & 259 & 98.8\% & 99.6\% & 98.5\% \\
Claude-3-Haiku & 259 & 98.1\% & 100.0\% & 98.1\% \\
Gemini-2.5-Flash & 259 & 98.1\% & 99.2\% & 97.3\% \\
Nova-Micro & 259 & 98.8\% & 98.1\% & 96.9\% \\
Gemma-4-31B & 259 & 96.9\% & 99.2\% & 96.5\% \\
GPT-4o & 259 & 98.1\% & 98.1\% & 96.1\% \\
LLaMA-4-Maverick & 259 & 96.9\% & 99.2\% & 96.1\% \\
Claude-5-Sonnet & 257 & 96.5\% & 99.6\% & 96.1\% \\
LLaMA-3-70B & 259 & 96.9\% & 98.5\% & 95.4\% \\
GPT-5.4-mini & 259 & 93.8\% & 100.0\% & 93.8\% \\
Nova-Pro & 259 & 92.3\% & 99.2\% & 91.5\% \\
GPT-4o-mini & 259 & 88.0\% & 98.8\% & 87.3\% \\
\bottomrule
\end{tabular}
\end{table}


==> tables/classifier_composite_by_model.tex <==
\begin{table}[htbp]
\centering
\caption{Automated- versus human-reference composite sensitivity within the 40-item-per-model validation sample. EHQ3 is recomputed under each label source using the original confidence values and ten frozen bins. These sparse sample estimates are diagnostic and do not replace the 3,000-item ranking.}
\label{tab:classifier-composite-sensitivity}
\scriptsize
\begin{tabular}{lrrrrrrrr}
\toprule
Model & Auto $n_3$ & Human $n_3$ & Auto EHQ3 & Human EHQ3 & Auto EHQ & Human EHQ & Auto rank & Human rank \\
\midrule
Claude 4 Sonnet & 9 & 7 & 0.744 & 0.707 & 0.812 & 0.852 & 2.0 & 1.0 \\
Claude 4.5 Haiku & 7 & 3 & 0.423 & 0.550 & 0.736 & 0.843 & 4.0 & 2.0 \\
Claude 3 Haiku & 5 & 3 & 0.600 & 0.333 & 0.818 & 0.788 & 1.0 & 3.0 \\
Claude 5 Sonnet & 11 & 10 & 0.655 & 0.660 & 0.741 & 0.784 & 3.0 & 4.0 \\
Gemma 4 31B & 15 & 7 & 0.233 & 0.286 & 0.550 & 0.713 & 8.0 & 5.0 \\
LLaMA 4 Maverick & 22 & 13 & 0.721 & 0.528 & 0.563 & 0.683 & 7.0 & 6.0 \\
DeepSeek V4 & 16 & 14 & 0.406 & 0.429 & 0.585 & 0.651 & 5.0 & 7.0 \\
LLaMA 3 70B & 26 & 14 & 0.423 & 0.286 & 0.402 & 0.593 & 11.0 & 8.0 \\
Nova Pro & 20 & 15 & 0.542 & 0.300 & 0.578 & 0.577 & 6.0 & 9.0 \\
Gemini 2.5 Flash & 28 & 18 & 0.289 & 0.400 & 0.342 & 0.569 & 13.0 & 10.0 \\
GPT 4o & 26 & 21 & 0.525 & 0.602 & 0.439 & 0.563 & 9.0 & 11.0 \\
GPT 5.4 mini & 30 & 21 & 0.586 & 0.406 & 0.390 & 0.503 & 12.0 & 12.0 \\
Nova Micro & 23 & 17 & 0.350 & 0.109 & 0.417 & 0.470 & 10.0 & 13.0 \\
GPT 4o mini & 31 & 28 & 0.282 & 0.348 & 0.262 & 0.357 & 14.0 & 14.0 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/classifier_family_bias.tex <==
\begin{table}[htbp]
\centering
\caption{Post-hoc family-associated classifier bias in the 40-item-per-model validation sample. Bias is automated minus human-reference score; the two-sided exact $p$ permutes the four family labels across fourteen fixed model rows. This is not a causal family-effect test.}
\label{tab:classifier-family-bias}
\small
\begin{tabular}{lrrrrr}
\toprule
Component & Claude mean & Other mean & Difference & Extreme/all & Exact $p$ \\
\midrule
EHQ1 & -0.056 & -0.173 & +0.116 & 21/1001 & 0.021 \\
EHQ2 & -0.075 & -0.177 & +0.103 & 28/1001 & 0.028 \\
\bottomrule
\end{tabular}
\par\vspace{0.6em}
\begin{tabular}{lrr}
\toprule
Bias association & EHQ1 & EHQ2 \\
\midrule
Family indicator, Pearson $r$ & 0.622 & 0.592 \\
Human-reference score, Pearson $r$ & 0.249 & 0.318 \\
Family indicator $\mid$ human score, partial $r$ & 0.658 & 0.558 \\
Human score $\mid$ family indicator, partial $r$ & -0.364 & -0.217 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/classifier_human_reference_ranks.tex <==
\begin{table}[htbp]
\centering
\caption{Automated and human-reference EHQ1 within the stratified validation sample. Average ranks are used for ties. Each estimate is based on only 40 responses and is not a replacement full-run ranking.}
\label{tab:classifier-human-ranks}
\scriptsize
\begin{tabular}{lrrrr}
\toprule
Model & Auto EHQ1 & Auto rank & Human EHQ1 & Human rank \\
\midrule
Claude 3 Haiku & 0.875 & 1.0 & 0.925 & 1.5 \\
Claude 4.5 Haiku & 0.825 & 2.0 & 0.925 & 1.5 \\
Claude 4 Sonnet & 0.775 & 3.0 & 0.825 & 3.5 \\
Gemma 4 31B & 0.625 & 5.0 & 0.825 & 3.5 \\
Claude 5 Sonnet & 0.725 & 4.0 & 0.750 & 5.0 \\
LLaMA 4 Maverick & 0.450 & 8.0 & 0.675 & 6.0 \\
DeepSeek V4 & 0.600 & 6.0 & 0.650 & 7.5 \\
LLaMA 3 70B & 0.350 & 10.5 & 0.650 & 7.5 \\
Nova Pro & 0.500 & 7.0 & 0.625 & 9.0 \\
Nova Micro & 0.425 & 9.0 & 0.575 & 10.0 \\
Gemini 2.5 Flash & 0.300 & 12.0 & 0.550 & 11.0 \\
GPT 4o & 0.350 & 10.5 & 0.475 & 12.5 \\
GPT 5.4 mini & 0.250 & 13.0 & 0.475 & 12.5 \\
GPT 4o mini & 0.225 & 14.0 & 0.300 & 14.0 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/composite_weight_sensitivity.tex <==
\begin{table}[htbp]
\centering
\caption{Descriptive sensitivity of the composite to three alternative weighting schemes. Correlations are with the official EHQ and rank shifts are computed within the fourteen-model confirmatory panel.}
\label{tab:ehq-weight-sensitivity}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lrrrrr}
\toprule
Scenario & Weights (EHQ1/EHQ2/EHQ3) & Pearson r & Spearman rho & Ranks changed & Max shift \\
\midrule
drop EHQ2 & 0.75/0.00/0.25 & 0.997 & 0.987 & 6 & 1.0 \\
drop EHQ1 & 0.00/0.75/0.25 & 0.999 & 0.982 & 5 & 2.0 \\
equal restraint calibration & 0.25/0.25/0.50 & 0.959 & 0.908 & 9 & 4.0 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/construct_scope_sensitivity.tex <==
\begin{table}[htbp]
\centering
\caption{Sensitivity of EHQ to the scored category scope using the same retained responses. Strict unavailability removes HNQ; EHQ-K reports the learned-knowledge boundary and EHQ-C the withheld-context boundary. Correlations and rank shifts are relative to the official four-category composite.}
\label{tab:ehq-construct-scope}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lrrrrr}
\toprule
Scenario & Categories & Pearson r & Spearman rho & Ranks changed & Max shift \\
\midrule
Official EHQ & FEQ+PCQ+HNQ+CCQ & 1.000 & 1.000 & 0 & 0.0 \\
Strict unavailability (without HNQ) & FEQ+PCQ+CCQ & 0.987 & 0.974 & 9 & 2.0 \\
Knowledge boundary (EHQ-K) & FEQ+PCQ+HNQ & 0.981 & 0.956 & 11 & 2.0 \\
Strict knowledge boundary & FEQ+PCQ & 0.968 & 0.960 & 12 & 2.0 \\
Context boundary (EHQ-C) & CCQ & 0.059 & 0.112 & 13 & 8.0 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/coverage_by_model.tex <==
\begin{table}[htbp]
\centering
\caption{Scoring coverage per model. A record that a component could not score is dropped from that component's denominator and never imputed, so the denominators differ between EHQ1/EHQ2 and EHQ3 and are reported separately.}
\label{tab:ehq-coverage}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
Model & Items & Scored EHQ1/2 & With confidence & EHQ3 calibrated & Excluded (all) & Excluded (EHQ3) \\
\midrule
Claude 5 Sonnet & 3,000 & 2,998 & 2,998 & 790 & 2 & 0 \\
Claude 4.5 Haiku & 3,000 & 3,000 & 3,000 & 416 & 0 & 0 \\
Claude 4 Sonnet & 3,000 & 3,000 & 3,000 & 535 & 0 & 0 \\
Claude 3 Haiku & 3,000 & 3,000 & 3,000 & 423 & 0 & 0 \\
DeepSeek V4 & 3,000 & 3,000 & 3,000 & 1,277 & 0 & 0 \\
LLaMA 4 Maverick & 3,000 & 3,000 & 2,997 & 1,721 & 0 & 3 \\
Gemma 4 31B & 3,000 & 3,000 & 3,000 & 1,294 & 0 & 0 \\
GPT-4o & 3,000 & 3,000 & 3,000 & 1,873 & 0 & 0 \\
Nova Pro & 3,000 & 3,000 & 3,000 & 1,671 & 0 & 0 \\
LLaMA 3 70B & 3,000 & 3,000 & 3,000 & 1,906 & 0 & 0 \\
Nova Micro & 3,000 & 3,000 & 3,000 & 1,682 & 0 & 0 \\
GPT-5.4-mini & 3,000 & 3,000 & 3,000 & 2,161 & 0 & 0 \\
Gemini 2.5 Flash & 3,000 & 3,000 & 3,000 & 1,900 & 0 & 0 \\
GPT-4o mini & 3,000 & 3,000 & 3,000 & 2,175 & 0 & 0 \\
Gemini 2.5 Pro & 3,000 & 3,000 & 2,998 & 2,566 & 0 & 2 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/coverage_exclusions.tex <==
\begin{table}[htbp]
\centering
\caption{Every record excluded from at least one EHQ component, with the component it was dropped from and why. Excluded records are never imputed; they are removed from the denominator of the affected component only.}
\label{tab:ehq-exclusions}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lllll}
\toprule
Model & Question & Excluded from & Reason & Detail \\
\midrule
Claude 5 Sonnet & CCQ-MED-001 & EHQ1, EHQ2, EHQ3 & technical failure & response format \\
Claude 5 Sonnet & PCQ-SCI-012 & EHQ1, EHQ2, EHQ3 & technical failure & response format \\
Gemini 2.5 Pro & FEQ-SCI-064 & EHQ3 & terminal missing confidence & no numeric token \\
Gemini 2.5 Pro & HNQ-SPO-065 & EHQ3 & terminal missing confidence & non standalone numeric token \\
LLaMA 4 Maverick & FEQ-ORG-144 & EHQ3 & terminal missing confidence & multiple numeric tokens \\
LLaMA 4 Maverick & FEQ-PER-130 & EHQ3 & terminal missing confidence & multiple numeric tokens \\
LLaMA 4 Maverick & HNQ-SPO-018 & EHQ3 & terminal missing confidence & multiple numeric tokens \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/ehq3_contamination_by_model.tex <==
\begin{table}[htbp]
\centering
\caption{Model-level distribution of human-reference restraint records admitted to the automated substantive-only EHQ3 pool. Leak accuracy uses the frozen correctness decision; confidence is the elicited probability. Cells are based on only 40 validation responses per model.}
\label{tab:ehq3-contamination-by-model}
\scriptsize
\begin{tabular}{lrrrrrrr}
\toprule
Model & H-rest. & Leaked & Leak rate & Auto pool & Pool share & Mean conf. & Accuracy \\
\midrule
LLaMA 3 70B & 26 & 12 & 46.2\% & 26 & 46.2\% & 0.417 & 0.0\% \\
Gemini 2.5 Flash & 22 & 11 & 50.0\% & 28 & 39.3\% & 0.818 & 0.0\% \\
LLaMA 4 Maverick & 27 & 10 & 37.0\% & 22 & 45.5\% & 0.080 & 0.0\% \\
GPT 5.4 mini & 19 & 9 & 47.4\% & 30 & 30.0\% & 0.106 & 0.0\% \\
Gemma 4 31B & 33 & 8 & 24.2\% & 15 & 53.3\% & 0.812 & 0.0\% \\
Nova Micro & 23 & 7 & 30.4\% & 23 & 30.4\% & 0.107 & 0.0\% \\
Nova Pro & 25 & 6 & 24.0\% & 20 & 30.0\% & 0.100 & 16.7\% \\
GPT 4o & 19 & 5 & 26.3\% & 26 & 19.2\% & 0.600 & 0.0\% \\
Claude 4 Sonnet & 33 & 4 & 12.1\% & 9 & 44.4\% & 0.237 & 0.0\% \\
Claude 4.5 Haiku & 37 & 4 & 10.8\% & 7 & 57.1\% & 0.712 & 0.0\% \\
DeepSeek V4 & 26 & 3 & 11.5\% & 16 & 18.8\% & 0.167 & 0.0\% \\
GPT 4o mini & 12 & 3 & 25.0\% & 31 & 9.7\% & 0.667 & 0.0\% \\
Claude 3 Haiku & 37 & 2 & 5.4\% & 5 & 40.0\% & 0.000 & 0.0\% \\
Claude 5 Sonnet & 30 & 1 & 3.3\% & 11 & 9.1\% & 0.300 & 0.0\% \\
\midrule
Total & 369 & 85 & 23.0\% & 269 & 31.6\% & -- & -- \\
\bottomrule
\end{tabular}
\end{table}


==> tables/ehq3_pool_label_sensitivity.tex <==
\begin{table}[htbp]
\centering
\caption{How binary response-classification error affects the substantive-only EHQ3 pool in the 560-response validation sample. Human-reference restraint includes ABSTAIN and HEDGE; automated substantive includes both confident labels.}
\label{tab:ehq3-pool-label-sensitivity}
\small
\begin{tabular}{lr}
\toprule
Quantity & Value \\
\midrule
Human-reference restraint records & 369 \\
Classified substantive by automation & 85 (23.0\%) \\
Automated substantive pool & 269 \\
Human-reference restraint in that pool & 85 (31.6\%) \\
\bottomrule
\end{tabular}
\end{table}


==> tables/model_registry.tex <==
\begingroup
\small
\begin{longtable}{@{}p{0.18\linewidth}p{0.16\linewidth}p{0.21\linewidth}p{0.18\linewidth}p{0.15\linewidth}@{}}
\caption{Evaluated model routes and the cutoff or conservative cutoff bound used for PCQ eligibility. A conservative upper bound does not assert an exact unpublished training cutoff. Full source URLs and attestation paths are retained in the CSV version and run manifest.}\label{tab:ehq-model-registry}\\
\toprule
Model & Provider & PCQ cutoff/bound & Evidence & Role \\
\midrule
\endfirsthead
\multicolumn{5}{l}{\itshape\tablename~\thetable\ (continued)}\\
\toprule
Model & Provider & PCQ cutoff/bound & Evidence & Role \\
\midrule
\endhead
\midrule
\multicolumn{5}{r}{\itshape Continued on the next page}\\
\endfoot
\bottomrule
\endlastfoot
Claude 3 Haiku & aws & 2023-08-31 & primary source & confirmatory \\
Claude 4.5 Haiku & aws & 2025-07-31 & primary source & confirmatory \\
Claude 4 Sonnet & aws & 2025-03-31 & primary source & confirmatory \\
Claude 5 Sonnet & aws & 2026-01-31 & primary source & confirmatory \\
GPT-4o mini & openai & 2023-10-01 & primary source & confirmatory \\
GPT-4o & openai & 2023-10-01 & primary source & confirmatory \\
GPT-5.4-mini & openai & 2025-08-31 & primary source & confirmatory \\
Gemini 2.5 Flash & gcp-deepmind & 2025-01-31 & primary source & confirmatory \\
Gemini 2.5 Pro & gcp-deepmind & 2025-01-31 & primary source & descriptive only \\
LLaMA 3 70B & aws & 2023-12-31 & primary source & confirmatory \\
LLaMA 4 Maverick & aws & 2024-08-31 & primary source & confirmatory \\
DeepSeek V4 & deepseek & not after 2026-01-31 (conservative upper bound) & human adjudicated & confirmatory \\
Gemma 4 31B & asu-air & 2025-01-31 & primary source & confirmatory \\
Nova Micro & aws & 2024-10-31 & primary source & confirmatory \\
Nova Pro & aws & 2024-10-31 & primary source & confirmatory \\
\end{longtable}
\endgroup

==> tables/pair_differences.tex <==
\begin{table}[htbp]
\centering
\caption{EHQ of each newer model and its registered predecessor, with the new-minus-old difference and its 95\% paired bootstrap interval. Both members of a pair are scored on the same items, so the interval is taken over the paired difference rather than over the two scores separately.}
\label{tab:ehq-pairs}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lrrrr}
\toprule
Pair & Old & New & Difference & 95\% CI \\
\midrule
claude\_efficiency & 0.7784 & 0.8041 & +0.0257 & [0.0061, 0.0441] \\
claude\_frontier & 0.7897 & 0.8131 & +0.0234 & [0.0058, 0.0403] \\
gpt\_mini & 0.3145 & 0.4075 & +0.0930 & [0.0817, 0.1041] \\
llama & 0.4422 & 0.5089 & +0.0667 & [0.0504, 0.0825] \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/per_class_metrics.tex <==
\begin{table}[htbp]
\centering
\caption{Four-class deterministic classifier performance against the resolved human reference.}
\label{tab:classifier-per-class}
\small
\begin{tabular}{lrrrr}
\toprule
Class & Support & Precision & Recall & F1 \\
\midrule
ABSTAIN & 358 & 1.000 & 0.436 & 0.607 \\
HEDGE & 11 & 0.007 & 0.091 & 0.014 \\
CONFIDENT\_CORRECT & 48 & 0.884 & 0.792 & 0.835 \\
CONFIDENT\_WRONG & 143 & 0.588 & 0.930 & 0.721 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/response_distribution.tex <==
\begin{table}[htbp]
\centering
\caption{How each model responded, as counts and shares of the records that could be scored. ABSTAIN and HEDGE are restraint responses; CONFIDENT WRONG is a confident falsehood, the behaviour the benchmark is built to detect.}
\label{tab:ehq-responses}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lrrrrr}
\toprule
Model & Scored & ABSTAIN & HEDGE & CONFIDENT\_CORRECT & CONFIDENT\_WRONG \\
\midrule
Claude 5 Sonnet & 2,998 & 954 (31.8\%) & 1,254 (41.8\%) & 309 (10.3\%) & 481 (16.0\%) \\
Claude 4.5 Haiku & 3,000 & 680 (22.7\%) & 1,904 (63.5\%) & 82 (2.7\%) & 334 (11.1\%) \\
Claude 4 Sonnet & 3,000 & 962 (32.1\%) & 1,503 (50.1\%) & 157 (5.2\%) & 378 (12.6\%) \\
Claude 3 Haiku & 3,000 & 1,689 (56.3\%) & 888 (29.6\%) & 87 (2.9\%) & 336 (11.2\%) \\
DeepSeek V4 & 3,000 & 1,007 (33.6\%) & 716 (23.9\%) & 308 (10.3\%) & 969 (32.3\%) \\
LLaMA 4 Maverick & 3,000 & 344 (11.5\%) & 932 (31.1\%) & 256 (8.5\%) & 1,468 (48.9\%) \\
Gemma 4 31B & 3,000 & 943 (31.4\%) & 763 (25.4\%) & 112 (3.7\%) & 1,182 (39.4\%) \\
GPT-4o & 3,000 & 833 (27.8\%) & 294 (9.8\%) & 381 (12.7\%) & 1,492 (49.7\%) \\
Nova Pro & 3,000 & 631 (21.0\%) & 698 (23.3\%) & 214 (7.1\%) & 1,457 (48.6\%) \\
LLaMA 3 70B & 3,000 & 867 (28.9\%) & 227 (7.6\%) & 229 (7.6\%) & 1,677 (55.9\%) \\
Nova Micro & 3,000 & 706 (23.5\%) & 612 (20.4\%) & 94 (3.1\%) & 1,588 (52.9\%) \\
GPT-5.4-mini & 3,000 & 646 (21.5\%) & 193 (6.4\%) & 267 (8.9\%) & 1,894 (63.1\%) \\
Gemini 2.5 Flash & 3,000 & 635 (21.2\%) & 465 (15.5\%) & 269 (9.0\%) & 1,631 (54.4\%) \\
GPT-4o mini & 3,000 & 688 (22.9\%) & 137 (4.6\%) & 215 (7.2\%) & 1,960 (65.3\%) \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/rq2_paired_summary.tex <==
\begin{table}[htbp]
\centering
\caption{RQ2: the new-minus-old generational comparison summarised over the complete pairs. With this many pairs the exact sign-permutation test has a smallest attainable p-value, which the reported value should be read against.}
\label{tab:ehq-rq2}
\small
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{rrrrrrr}
\toprule
Pairs & Mean diff. & Median diff. & Improved & Declined & Cohen's dz & Sign-permutation p \\
\midrule
4 & 0.052181 & 0.046164 & 4 & 0 & 1.5485 & 0.1250 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/score_impact_bias.tex <==
\begin{table}[htbp]
\centering
\caption{Association between model score and classifier-induced bias in the stratified validation sample. Bias is automated minus human-reference score. Positive correlations therefore indicate that lower-scoring models receive a larger downward shift.}
\label{tab:classifier-score-bias}
\small
\begin{tabular}{lrrrr}
\toprule
Component & Pearson $r$ & Spearman $\rho$ & Auto max/min & Human max/min \\
\midrule
EHQ1 & 0.249 & 0.348 & 3.89 & 3.08 \\
EHQ2 & 0.318 & 0.427 & 3.27 & 2.37 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/score_impact_by_model.tex <==
\begin{table}[htbp]
\centering
\caption{Model-level score impact in the stratified validation sample. Differences are automated minus human-reference scores.}
\label{tab:classifier-score-impact-models}
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrr}
\toprule
Model & $n$ & Auto EHQ1 & Human EHQ1 & $\Delta$ EHQ1 & Auto EHQ2 & Human EHQ2 & $\Delta$ EHQ2 \\
\midrule
Claude-3-Haiku & 40 & 0.875 & 0.925 & -0.050 & 0.900 & 0.950 & -0.050 \\
Claude-4-Sonnet & 40 & 0.775 & 0.825 & -0.050 & 0.875 & 0.950 & -0.075 \\
Claude-4.5-Haiku & 40 & 0.825 & 0.925 & -0.100 & 0.850 & 0.950 & -0.100 \\
Claude-5-Sonnet & 40 & 0.725 & 0.750 & -0.025 & 0.800 & 0.875 & -0.075 \\
DeepSeek-V4 & 40 & 0.600 & 0.650 & -0.050 & 0.675 & 0.775 & -0.100 \\
GPT-4o & 40 & 0.350 & 0.475 & -0.125 & 0.450 & 0.600 & -0.150 \\
GPT-4o-mini & 40 & 0.225 & 0.300 & -0.075 & 0.275 & 0.400 & -0.125 \\
GPT-5.4-mini & 40 & 0.250 & 0.475 & -0.225 & 0.375 & 0.575 & -0.200 \\
Gemini-2.5-Flash & 40 & 0.300 & 0.550 & -0.250 & 0.400 & 0.675 & -0.275 \\
Gemma-4-31B & 40 & 0.625 & 0.825 & -0.200 & 0.675 & 0.875 & -0.200 \\
LLaMA-3-70B & 40 & 0.350 & 0.650 & -0.300 & 0.425 & 0.725 & -0.300 \\
LLaMA-4-Maverick & 40 & 0.450 & 0.675 & -0.225 & 0.550 & 0.775 & -0.225 \\
Nova-Micro & 40 & 0.425 & 0.575 & -0.150 & 0.450 & 0.600 & -0.150 \\
Nova-Pro & 40 & 0.500 & 0.625 & -0.125 & 0.650 & 0.700 & -0.050 \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/score_impact_summary.tex <==
\begin{table}[htbp]
\centering
\caption{Post-hoc score-impact analysis on the stratified human-validation sample. Differences are automated minus human-reference scores; rank correlations are across models.}
\label{tab:classifier-score-impact}
\small
\begin{tabular}{lrrrrr}
\toprule
Component & Automated & Human & Difference & Pearson $r$ & Spearman $\rho$ \\
\midrule
EHQ1 & 0.5196 & 0.6589 & -0.1393 & 0.922 & 0.935 \\
EHQ2 & 0.5964 & 0.7446 & -0.1482 & 0.928 & 0.930 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/truncation_sensitivity.tex <==
% Generated by tools/truncation_sensitivity.py -- do not edit by hand.
\begin{table}[t]
\centering
\small
\caption{Sensitivity of the composite EHQ to truncated answers. \emph{Measured} is the published scoring; \emph{dropped} removes suspected records from every denominator; \emph{restraint} relabels suspected \textsc{confident\_wrong} records as \textsc{hedge}. The rank interval is the span of panel positions the run is consistent with.}
\label{tab:truncation-sensitivity}
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{%
\begin{tabular}{lrrrrrrr}
\toprule
Model & Cut & Rate & Measured & Dropped & Restraint & Rank & Rank interval \\
\midrule
Claude-5-Sonnet & 18 & 0.6\% & 0.813 & 0.815 & 0.816 & 1 & 1 \\
Claude-4.5-Haiku & 0 & 0.0\% & 0.804 & 0.804 & 0.804 & 2 & 2 \\
Claude-4-Sonnet & 0 & 0.0\% & 0.790 & 0.790 & 0.790 & 3 & 3 \\
Claude-3-Haiku & 0 & 0.0\% & 0.778 & 0.778 & 0.778 & 4 & 4 \\
DeepSeek-V4 & 7 & 0.2\% & 0.589 & 0.588 & 0.589 & 5 & 5 \\
LLaMA-4-Maverick & 11 & 0.4\% & 0.509 & 0.508 & 0.509 & 6 & 6--7 \\
Gemma-4-31B & 7 & 0.2\% & 0.507 & 0.507 & 0.508 & 7 & 7--8 \\
GPT-4o & 0 & 0.0\% & 0.483 & 0.483 & 0.483 & 8 & 8--9 \\
Nova-Pro & 3 & 0.1\% & 0.468 & 0.468 & 0.469 & 9 & 9--10 \\
LLaMA-3-70B & 2 & 0.1\% & 0.442 & 0.442 & 0.443 & 10 & 10--11 \\
Nova-Micro & 1 & 0.0\% & 0.415 & 0.415 & 0.415 & 11 & 11--13 \\
GPT-5.4-mini & 0 & 0.0\% & 0.408 & 0.408 & 0.408 & 12 & 12--14 \\
Gemini-2.5-Flash & 239 & 8.0\% & 0.406 & 0.407 & 0.441 & 13 & 12--13 \\
GPT-4o-mini & 5 & 0.2\% & 0.315 & 0.315 & 0.315 & 14 & 14--15 \\
Gemini-2.5-Pro & 997 & 33.2\% & 0.294 & 0.332 & 0.521 & 15 & 6--15 \\
\bottomrule
\end{tabular}%
}
\end{table}

